Rethinking the 67 Hz QPO in GRS 1915+105: type-C QPOs at the innermost stable circular orbit

Context. The study of Quasi-Periodic Oscillations (QPO) at low and high frequency in the variability of the high-energy emission from black-hole binaries and their physical interpretation in terms of signatures of General Relativity in the strong-field regime. Aims. To understand the nature of the 67 Hz QPOs observed in the X-ray emission of the peculiar black-hole binary GRS 1915+105 within the general classification of QPO and to determine the spin of the black hole in the system by applying the Relativistic Precession Model (RPM). Methods. Within the RPM, the only relativistic frequency that is stable in time over a large range of accretion rates and can be as low as 67 Hz (for a black-hole mass as measured dynamically) is the Lense-Thirring frequency at the Innermost Stable Circular Orbit (ISCO). In the application of the model, this corresponds to type-C QPOs. Under this assumption, it is possible to measure the spin of the black hole. We re-analysed a large number of RossiXTE observations to check whether other timing features confirm this hypothesis. Results. The identification of the 67 Hz QPO as the Lense-Thirring frequency at ISCO yields a value of 0.706 +/- 0.034 for the black hole spin. With this spin, the only two QPO detections at higher frequencies available in the literature are consistent with being orbital frequencies at a radius outside ISCO. The high-frequency bumps often observed at frequencies between 10 and 200 Hz follow the correlation expected for orbital and periastron-precession frequencies at even larger radii.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\apjs{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\araa{Annual Reviews}
\def\apss{Ap\&SS}
\def\atel{The Astronomer's Telegram}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\ssr{Space Science Reviews}
\def\prd{Physical Review D}
\def\pasp{Publications of the Astronomical Society of the Pacific}
\def\na{New Astronomy}
